Double Perturbation: On the Robustness of Robustness and Counterfactual Bias Evaluation

Robustness and counterfactual bias are usually evaluated on a test dataset. However, are these evaluations robust? If the test dataset is perturbed slightly, will the evaluation results keep the same? In this paper, we propose a "double perturbation" framework to uncover model weaknesses beyond the test dataset. The framework first perturbs the test dataset to construct abundant natural sentences similar to the test data, and then diagnoses the prediction change regarding a single-word substitution. We apply this framework to study two perturbation-based approaches that are used to analyze models' robustness and counterfactual bias in English. (1) For robustness, we focus on synonym substitutions and identify vulnerable examples where prediction can be altered. Our proposed attack attains high success rates (96.0%-99.8%) in finding vulnerable examples on both original and robustly trained CNNs and Transformers. (2) For counterfactual bias, we focus on substituting demographic tokens (e.g., gender, race) and measure the shift of the expected prediction among constructed sentences. Our method is able to reveal the hidden model biases not directly shown in the test dataset. Our code is available at https://github.com/chong-z/nlp-second-order-attack.

==> buffer.tex <==

\todo{Old introduction, add to related work:}
Contemporary NLP models are vulnerable to adversarial perturbations, where a seemingly label-preserving transformation can alter the model prediction.
For instance, the model can be fooled by synonym substitutions \citep{alzantot-etal-2018-generating, Garg2020BAEBA, li2020bertattack, Zang_2020, jin2019bert, Cheng_2020}, character-level substitutions \citep{ebrahimi-etal-2018-hotflip, Gao_2018}, appending or prepending text \citep{Jia2017AdversarialEF}, paraphrasing \citep{Iyyer2018AdversarialEG, ribeiro-etal-2018-semantically}, input reduction \citep{Feng_2018}, and text from generative adversarial networks \citep{zhao2018generating}.

Past works evaluate robustness on a fixed test dataset (we refer as \emph{\fo robustness}), where they consider the model robust if most examples from the test dataset are resistant to adversarial attacks (e.g., measured by accuracy under attack).
% by the ratio of test examples that are robust under attack (e.g., adversarial accuracy or certified accuracy), and mitigated the problem on a fixed test dataset.
% we refer as \emph{\fo robustness}.
% Past work mitigated the problem on a fixed test dataset, but it is still unclear whether the model is truly robust under the wide range of real world inputs. 
For instance, \citet{alzantot-etal-2018-generating} experimented adversarial training \citep{madry2018towards} on natural language models.
\citet{Jia2019CertifiedRT, Huang_2019} applied verifiable training through Interval Bound Propagation (IBP) on label-preserving symbol substitutions and achieved $\sim$75\% adversarial accuracy on CNN and LSTM. 
\citet{Shi2020Robustness} certified the robustness for Transformers and provided a much tighter bound than IBP. \citet{xu2020automatic} further improved the algorithm and provided robustness verification on general computational graphs.
However, real world inputs are manifold and \fo robustness may give a false sense of security. \cref{fig:intro} provides an example where $\tilde{x}_0 \notin \cX_\text{test}$ is a valid input example to $f$, however it may be vulnerable to adversarial attacks even if $f$ is certified robust.
\todo{Move to related word and focus more on our work.}

In this paper we propose the concept of \emph{\so robustness} where we evaluate model robustness on the augmented dataset along the $\ell_0$ norm ball. We consider an example \so robust if all natural examples within its $\ell_0$ norm ball are \fo robust. The augmentation process is automatic and covers a wide variety of examples compared to conventional label-preserving transformations (e.g., synonym substitutions).
To better illustrate why $\tilde{x}_0$ in \cref{fig:intro} is not \fo robust we plot the illustrated decision boundary in \cref{fig:circle}. Here $x_0 \in \cX_\text{test}$ is certified \fo robust (diamond area) but not \so robust (circle area) since $\tilde{x}_0$ and $\tilde{x}_1$ are not \fo robust. As shown we have an adversarial example $\tilde{x}_0'$ for $\tilde{x}_0$ where $f(\tilde{x}_0') \ne f(\tilde{x}_0)$, and their only difference is a single pair of synonyms (\w{film}, \w{movie}).
\jy{btw, where is $x_2$ in Fig.1?}\chong{Sorry for the confusion, I updated the figure with correct labels.}
\todo{Move definition to next sec}

% , where for an example such as \w{a sometimes tedious film.} the model prediction is certified to remain the same if the attacker changes \w{tedious} to \w{boring}, or \w{film} to \w{movie}. However, it is unclear whether the model is robust after non-label-preserving transformations such as \w{a sometimes \textit{attractive} film.} since we don't know the ground truth label.


Additionally, we observe gender bias where the model takes specious gender related identities as features in making decisions, and such bias often correspond to the training dataset. Such bias is undesired since the model is not intended to discriminate between the gender of people, and we consider it as a special form of model vulnerability.\jy{I think it's better to move this definition to the beginning of the paragraph..}\chong{Moved to the beginning, thanks for the suggestions!} In this work our definition is: \emph{A model contains gender bias if the expected prediction for inputs containing male identities is significantly higher or lower from inputs containing female identities.}
Past work studied this type of specious correlation: \citet{dixon2018measuring} showed that the imbalances in training data can lead to unintended bias, where the resulting model may give unreasonably high toxicity scores to sentences containing certain identity terms such as \w{I am a gay man}. \citet{park-etal-2018-reducing} showed that abusive language detection models rank sentences containing female noun phrases to be more \w{sexist} than those containing male noun phrases. \citet{Zhao_2017} demonstrated that gender bias in the training dataset will be further amplified in the resulting model.
We provide a case study for gender bias in \cref{sec:bias}.



==> tables/attack_lm_score.tex <==
\robusttable{\makecell{LM Score\\Difference}}{
         bow &                 -1.03 &          0.22 &     0.19 &            0.22 \\
         cnn &                 -0.97 &          0.09 &     0.24 &            0.25 \\
        lstm &                 -0.83 &          0.24 &     0.22 &            0.21 \\
 transformer &                 -0.98 &          0.06 &     0.24 &            0.24 \\
}{
         bow &                 -0.59 &          0.27 &     0.23 &            0.29 \\
         cnn &                 -0.75 &          0.18 &     0.20 &            0.23 \\
        lstm &                 -0.88 &          0.23 &     0.32 &            0.27 \\
 transformer &                 -0.88 &          0.11 &     0.27 &            0.24 \\
}



==> tables/attack_stats.tex <==
\begin{tabular}{lcccc|cccc|cccc}
\toprule
      & \multicolumn{4}{c|}{\textbf{Attack Success Rate - mean \%}} & \multicolumn{4}{c|}{\textbf{GPT-2 Perplexity Increase - median}} & \multicolumn{4}{c}{\textbf{$\ell_0$ Norm Distance - mean}} \\
             &             Genetic & BAE & \makecell{SO-Enum} & \makecell{SO-Beam} &               Genetic &  BAE & \makecell{SO-Enum} & \makecell{SO-Beam} &        Genetic &   BAE & \makecell{SO-Enum} & \makecell{SO-Beam} \\
\midrule
\multicolumn{2}{l}{\textbf{Base Models:}} \\
         BoW &                   57.0 &  69.7 &    95.3 &    \first{99.7} &               86 &  49 &   \first{13} &   15 &                    3.3 &           1.6 &      \first{1.1} &             1.2 \\
         CNN &                   62.0 &  71.0 &    95.3 &    \first{99.8} &              117 &  41 &   \first{18} &  \first{18} &                    3.0 &           1.5 &      \first{1.1} &             1.2 \\
        LSTM &                   60.0 &  68.3 &    95.8 &    \first{99.5} &               99 &  46 &   \first{16} &   17 &                    2.9 &           1.6 &      \first{1.1} &             1.2 \\
 Transformer &                   73.0 &  74.3 &    95.4 &    \first{98.0} &               75 &  41 &   \first{11} &   12 &                    2.8 &           1.4 &      \first{1.0} &             1.1 \\
   BERT-Base &                   41.0 &  61.5 &    94.3 &    \first{98.7} &              137 &  54 &  \first{39} &  40 &                    3.4 &           1.6 &      \first{1.3} &             1.4 \\
\multicolumn{2}{l}{\textbf{Robust Models:}} \\
         BoW &                   28.0 &  63.1 &    81.5 &    \first{88.4} &                51 &  46 &  \first{26} &  27 &                    2.4 &           1.5 &      \first{1.2} &             1.4 \\
         CNN &                   23.0 &  64.4 &    91.0 &    \first{96.0} &               92 &  48 &   \first{22} &   23 &                    2.7 &           1.5 &      \first{1.2} &             1.3 \\
        LSTM &                   24.0 &  61.0 &    62.9 &    \first{77.5} &               73 &  50 &  \first{27} &  39 &                    2.5 &           1.6 &      \first{1.3} &             1.8 \\
 Transformer &                   56.0 &  71.6 &    91.2 &    \first{96.2} &               58 &  40 &   \first{20} &   21 &                    2.8 &           1.4 &      \first{1.2} &             1.3 \\
\bottomrule
\end{tabular}

==> tables/attack_stats_bk_withbold.tex <==
\begin{tabular}{lcccc|cccc|cccc}
\toprule
      & \multicolumn{4}{c|}{\textbf{Attack Success Rate - mean \%}} & \multicolumn{4}{c|}{\textbf{GPT-2 Perplexity Increase - median\footnotemark}} & \multicolumn{4}{c}{\textbf{$\ell_0$ Norm Distance - mean}} \\
             &             Genetic & BAE & \makecell{SO-Enum} & \makecell{SO-Beam} &               Genetic &  BAE & \makecell{SO-Enum} & \makecell{SO-Beam} &        Genetic &   BAE & \makecell{SO-Enum} & \makecell{SO-Beam} \\
\midrule
\multicolumn{2}{l}{\textbf{Base Models:}} \\
         BoW &                   57.0 &  69.7 &    95.3 &    \textbf{99.7} &               86 &  49 &   \textbf{13} &   15 &                    3.3 &           1.6 &      \textbf{1.1} &             1.2 \\
         CNN &                   62.0 &  71.0 &    95.3 &    \textbf{99.8} &              117 &  41 &   \textbf{18} &  \textbf{18} &                    3.0 &           1.5 &      \textbf{1.1} &             1.2 \\
        LSTM &                   60.0 &  68.3 &    95.8 &    \textbf{99.5} &               99 &  46 &   \textbf{16} &   17 &                    2.9 &           1.6 &      \textbf{1.1} &             1.2 \\
 Transformer &                   73.0 &  74.3 &    95.4 &    \textbf{98.0} &               75 &  41 &   \textbf{11} &   12 &                    2.8 &           1.4 &      \textbf{1.0} &             1.1 \\
   BERT-Base &                   41.0 &  61.5 &    94.3 &    \textbf{98.7} &              137 &  54 &  \textbf{39} &  40 &                    3.4 &           1.6 &      \textbf{1.3} &             1.4 \\
\multicolumn{2}{l}{\textbf{Robust Models:}} \\
         BoW &                   28.0 &  63.1 &    81.5 &    \textbf{88.4} &                51 &  46 &  \textbf{26} &  27 &                    2.4 &           1.5 &      \textbf{1.2} &             1.4 \\
         CNN &                   23.0 &  64.4 &    91.0 &    \textbf{96.0} &               92 &  48 &   \textbf{22} &   23 &                    2.7 &           1.5 &      \textbf{1.2} &             1.3 \\
        LSTM &                   24.0 &  61.0 &    62.9 &    \textbf{77.5} &               73 &  50 &  \textbf{27} &  39 &                    2.5 &           1.6 &      \textbf{1.3} &             1.8 \\
 Transformer &                   56.0 &  71.6 &    91.2 &    \textbf{96.2} &               58 &  40 &   \textbf{20} &   21 &                    2.8 &           1.4 &      \textbf{1.2} &             1.3 \\
\bottomrule
\end{tabular}

==> tables/bert_score_diff.tex <==
\begin{tabular}{lcccc}
\toprule
              & \multicolumn{4}{c}{\textbf{BERT Score Increase}} \\
                   & Genetic & BAE & SO-Enum & SO-Beam \\
\midrule
\multicolumn{2}{l}{\textbf{Base Models:}} \\
         BoW &      -0.98 &  0.12 &    \first{0.24} &    0.23 \\
         CNN &      -0.89 &  0.11 &    \first{0.20} &    \first{0.20} \\
        LSTM &      -0.86 &  0.13 &    0.19 &    \first{0.21} \\
 Transformer &      -1.01 &  0.05 &    0.23 &    \first{0.24} \\
   BERT-base &      -1.09 &  0.04 &    \first{0.18} &    \first{0.18} \\
\multicolumn{2}{l}{\textbf{Robust Models:}} \\
         BoW &      -0.65 &  0.17 &    0.20 &    \first{0.21} \\
         CNN &      -0.73 &  0.14 &    0.18 &    \first{0.22} \\
        LSTM &      -0.82 &  0.21 &    \first{0.23} &    \first{0.23} \\
 Transformer &      -1.00 &  0.06 &    0.26 &    \first{0.27} \\
\bottomrule
\end{tabular}

==> tables/genetic_on_vulnerable.tex <==
\begin{tabular}{lccccccc}
\toprule
             & \multicolumn{3}{c}{\textbf{Genetic on Test Set}} & \multicolumn{4}{c}{\textbf{Attack after \sob}} \\
      & \makecell{Ori./Vul.\\PPL} & \makecell{Adv.\\PPL} & \makecell{$\ell_0$} & \makecell{Ori.\\PPL} & \makecell{Vul.\\PPL} & \makecell{Adv.\\PPL} & \makecell{$\ell_0$} \\
\midrule
\multicolumn{2}{l}{\textbf{Base Models:}} \\
         BoW &      145 &       258 &    3.3  &   163 &           187 &           283 &     1.0 \\
         CNN &      146 &       282 &    3.0  &   163 &           205 &           267 &     1.0 \\
        LSTM &      131 &       238 &    2.9  &   163 &           187 &           263 &     1.0 \\
 Transformer &      137 &       232 &    2.8  &   158 &           181 &           255 &     1.0 \\
   BERT-base &      201 &       342 &    3.4  &   163 &           212 &           279 &     1.0 \\
\multicolumn{2}{l}{\textbf{Robust Models:}} \\
         BoW &      132 &       177 &    2.4  &   163 &           223 &           261 &     1.0 \\
         CNN &      136 &       236 &    2.7  &   163 &           198 &           237 &     1.0 \\
        LSTM &      163 &       267 &    2.5  &   181 &           246 &           315 &     1.0 \\
 Transformer &      118 &       200 &    2.8  &   160 &           212 &           232 &     1.0 \\
\bottomrule
\end{tabular}



==> tables/model_acc.tex <==
\begin{tabular}{lcc}
\toprule
 & Clean Acc. & Cert Acc. \\
\midrule
\multicolumn{3}{l}{\textbf{Standard models}} \\
bow & 81.4\% & 0.3\% \\
cnn & 82.5\% & 0.1\% \\
lstm & 81.7\% & 0.0\% \\
transformer & 82.1\% & 0.0\% \\
\midrule
\multicolumn{3}{l}{\textbf{\Fo robust models}}\\
bow & 79.5\% & 49.8\% \\
cnn & 77.6\% & 51.2\% \\
lstm & 78.5\% & 47.9\% \\
transformer & 81.8\% & 77.1\% \\
\bottomrule
\end{tabular}

==> tables/num_perturb_words.tex <==
\begin{tabular}{lcccc}
\toprule
              & \multicolumn{4}{c}{\textbf{Num of Perturbed Words}} \\
                   & Genetic & BAE & SO-Enum & SO-Beam \\
\midrule
\multicolumn{2}{l}{\textbf{Base Models:}} \\
               BoW &                   3.3 &           1.6 &      \textbf{1.1} &             1.2 \\
               CNN &                   3.0 &           1.5 &      \textbf{1.1} &             1.2 \\
              LSTM &                   2.9 &           1.6 &      \textbf{1.1} &             1.2 \\
       Transformer &                   2.8 &           1.4 &      \textbf{1.0} &             1.1 \\
         BERT-Base &                   3.4 &           1.6 &      \textbf{1.3} &             1.4 \\
\multicolumn{2}{l}{\textbf{Robust Models:}} \\
               BoW &                   2.4 &           1.5 &      \textbf{1.2} &             1.4 \\
               CNN &                   2.7 &           1.5 &      \textbf{1.2} &             1.3 \\
              LSTM &                   2.5 &           1.6 &      \textbf{1.3} &             1.8 \\
       Transformer &                   2.8 &           1.4 &      \textbf{1.2} &             1.3 \\
\bottomrule
\end{tabular}

==> tables/threat-model-sample.tex <==
\resizebox{1\columnwidth}{!}{
\begin{tabular}{rlrl}
\toprule
\multicolumn{2}{c}{Initial Victim Example} & \multicolumn{2}{c}{Adversarial Examples} \\ \midrule
$x_0$ & a sometimes tedious film. & $x_0'$ & a sometimes tedious \textbf{movie}. \\
\midrule
\multicolumn{2}{c}{Examples in $\text{Ball}_{1}(x_0)$} & \multicolumn{2}{c}{Adversarial Examples} \\ \midrule
$\tilde{x}_0$ &a sometimes attractive film. & $\tilde{x}_0'$ & a sometimes attractive \textbf{movie}. \\
$\tilde{x}_1$ &a never tedious film. & $\tilde{x}_1'$ & a never tedious \textbf{movie}. \\
% $\tilde{x}_2$ & a sometimes tedious movie. & $\tilde{x}_2'$ & a sometimes tedious \textbf{film}. \\
\bottomrule
\end{tabular}
}


==> tables/use.tex <==
\begin{tabular}{lcccc}
\toprule
              & \multicolumn{4}{c}{\textbf{USE Cosine Similarity}} \\
                   & Genetic & BAE & SO-Enum & SO-Beam \\
\midrule
\multicolumn{2}{l}{\textbf{Base Models:}} \\
               BoW &                   0.83 &  0.83 &    \first{0.89} &    \first{0.89} \\
               CNN &                   0.83 &  0.84 &    0.88 &    \first{0.89} \\
              LSTM &                   0.84 &  0.84 &    \first{0.88} &    \first{0.88} \\
       Transformer &                   0.84 &  0.85 &    \first{0.89} &    \first{0.89} \\
         BERT-base &                   0.83 &  0.84 &    \first{0.89} &    \first{0.89} \\
\multicolumn{2}{l}{\textbf{Robust Models:}} \\
               BoW &                   0.86 &  0.84 &    \first{0.89} &    \first{0.89} \\
               CNN &                   0.83 &  0.83 &    \first{0.89} &    \first{0.89} \\
              LSTM &                   0.84 &  0.82 &    0.87 &    \first{0.88} \\
       Transformer &                   0.84 &  0.84 &    \first{0.89} &    \first{0.89} \\
\bottomrule
\end{tabular}
